RandAugment: Practical automated data augmentation with a reduced search space

Recent work has shown that data augmentation has the potential to significantly improve the generalization of deep learning models. Recently, automated augmentation strategies have led to state-of-the-art results in image classification and object detection. While these strategies were optimized for improving validation accuracy, they also led to state-of-the-art results in semi-supervised learning and improved robustness to common corruptions of images. An obstacle to a large-scale adoption of these methods is a separate search phase which increases the training complexity and may substantially increase the computational cost. Additionally, due to the separate search phase, these approaches are unable to adjust the regularization strength based on model or dataset size. Automated augmentation policies are often found by training small models on small datasets and subsequently applied to train larger models. In this work, we remove both of these obstacles. RandAugment has a significantly reduced search space which allows it to be trained on the target task with no need for a separate proxy task. Furthermore, due to the parameterization, the regularization strength may be tailored to different model and dataset sizes. RandAugment can be used uniformly across different tasks and datasets and works out of the box, matching or surpassing all previous automated augmentation approaches on CIFAR-10/100, SVHN, and ImageNet. On the ImageNet dataset we achieve 85.0% accuracy, a 0.6% increase over the previous state-of-the-art and 1.0% increase over baseline augmentation. On object detection, RandAugment leads to 1.0-1.3% improvement over baseline augmentation, and is within 0.3% mAP of AutoAugment on COCO. Finally, due to its interpretable hyperparameter, RandAugment may be used to investigate the role of data augmentation with varying model and dataset size. Code is available online.

==> intro_table_old.tex <==
\begin{table}[t]
\scriptsize
\begin{tabular}{l|cc|cc|cc|cc}
          & \multicolumn{2}{c|}{\textbf{CIFAR-10}} & \multicolumn{2}{c|}{\textbf{SVHN}} & \multicolumn{2}{c|}{\textbf{ImageNet}} & \multicolumn{2}{c}{\textbf{ImageNet}} \\
          & \multicolumn{2}{c|}{PyramidNet}        & \multicolumn{2}{c|}{Wide-ResNet}   & \multicolumn{2}{c|}{ResNet-50}         & \multicolumn{2}{c}{EfficientNet-B7}      \\ \hline
          & cost              & acc.              & cost            & acc.            & cost              & acc.              & cost              & acc.              \\ \hline
Baseline & 0 & 97.3 & 0 & 98.5 & 0 & 76.3 & 0 & 84.0 \\
\hline
AA        & 5K              & 98.5              & 1K            & 98.9            & 15K             & 77.6             & 15K             & 84.4            \\
Fast AA   & 3.5               & 98.3              & 1.5             & 98.8            & 450               & 77.6             & -                 & -                  \\
PBA       & 5.0               & 98.5              & 1.0             & 98.9            & -                 & -                  & -                 & -                  \\
RA (ours) & 0                 & 98.5              & 0               & 99.0            & 0                 & 77.6             & 0                 & 85.0             \\
\end{tabular}
\vspace{0.2cm}
\caption{\textbf{RandAugment matches or exceeds predictive performance of other augmentation methods but with zero search cost on a separate proxy task.} We report the number of GPU hours spent on the learned augmentation search and the test accuracy achieved for AutoAugment (AA) \cite{cubuk2018autoaugment}, Fast AutoAugment \cite{lim2019fast}, Population Based Augmentation (PBA) \cite{ho2019population} and the proposed RandAugment (RA) for CIFAR-10~\cite{krizhevsky2009learning}, SVHN~\cite{netzer2011reading} and ImageNet~\cite{imagenet2009} classification tasks. Computational cost is reported as the number of GPU hours expended for identifying the augmentation policy in a separate search phase on a proxy task. The error rate is reported as a percentage on a cross-validated validation or test split. Dash indicates that results are not available.}
\label{tab:summary_results}  
\end{table}
